Spontaneous Symmetry Breaking of an Optical Polarization State in a Polarization-Selective Nonlinear Resonator

We exploit polarization self-rotation in atomic rubidium vapor to observe spontaneous symmetry breaking and bistability of polarization patterns. We pump the vapor cell with horizontally polarized light while the vertical polarization, which is initially in the vacuum state, is resonated in a ring cavity. Vacuum fluctuations in this mode experience cumulative gain due to the compound action of amplification due to the self-rotation and feedback through the resonator, eventually acquiring a macroscopic magnitude akin to an optical parametric oscillator. The randomness of these fluctuations results in a bistable, random macroscopic polarization pattern at the output. We propose utilizing this mechanism to simulate Ising-like interaction between multiple spatial modes and as a basis for a fully optical coherent Ising machine.

==> deleted_parts_in_case_we_will_decide_to_use_them.tex <==

%скопировал из сащиной статьи. Назание лаера и длинну волны с мозностью поменял на наше. Дальше ничего не менял
%The scheme of our experimental setup is shown in Fig. 1. A external cavity diode laser (Vitawave ECDL-7950R) delivered $\approx 50 \mathrm{~mW}$ of optical power in a single mode at a wavelength of $794.7 \mathrm{~nm}$, tunable across the rubidium $D 1$ line. The beam was shaped with a pair of cylindrical lenses and a Glan prism purified the linear polarization. The beam was focused by a lens $(f=200 \mathrm{~mm})$ into a heated $75-\mathrm{mm}$ rubidium cell filled with the nearly pure isotope ${ }^{85} \mathrm{Rb}$. With a focal beam diameter of $600 \mu \mathrm{m}$, we operated in a high saturation regime.
%To determine the polarization self-rotation parameter $g l$,% я бы тут не писал про gl мб
%a fine-adjustable $\lambda / 4$ plate was placed in front of the cell. Its rotation angle in radians was equal to the generated ellipticity $\epsilon$. The outputs of the second PBS were directly fed into two photodiodes. A $\lambda / 2$ plate placed after the cell was adjusted so that the dc photodiode signals $S_1$ and $S_2$ were exactly equal when the laser was detuned far from the resonance. This "balanced polarimeter" was sensitive to the polarization ellipse rotation while being insensitive to mined from the photodiode signal difference:

стояло на 251 строке:
%Here we describe the process in more details.
%Horizontally polarised pump $\mathcal{E} = \mathcal{E}_H \equiv X_H $ gets a vertically polarised component because of fluctuations. In terms of quadratures the newly obtained component can be described as $\mathcal{E}_V = X_V + i P_V$,
%where X-quadrature is in phase with the pump, and P-quadrature is shifted in phase by $ \pi / 2 $. In that notation, ellipticity of light in the first order will be described by equation \ref{eq:ell}.

%Metamorphosis of vertically polarised component is presented in figure \ref{fig:phasespace}. %say about phase plane?

%\begin{figure}[h]
%\begin{center}
 % \includegraphics[width=.41\linewidth]{bist_img/0.png}
% \includegraphics[width=.41\linewidth]{bist_img/1.png}\\
 % \includegraphics[width=.41\linewidth]{bist_img/2.png}
 % \includegraphics[width=.41\linewidth]{bist_img/3.png}
% \end{center}
%\label{fig:phasespace}
%\end{figure} 

%(a) shows the phase space of vertical polarisation before interaction with nonlinear medium. As light goes through vapour cell, weak self-rotation occurs (fig. (b)). If we somehow add a relative phase shift between vertical and horizontal components, it will result in rotation of vertical polarisation state in phase plane, as shown in (c). It can lead to increase of $P_V$ value, or in other words, to higher ellipticity. Sending this new signal into rubidium cell again, one can observe more prominent self-rotation (d).

%Taking into account that the initial microscopic ellipticity caused by fluctuations can have an arbitrary helicity, the final direction of the macroscopic self-rotation of the polarization ellipse appears to be random. (Fig. 5)



==> old_bibliography.tex <==
% \begin{thebibliography}{99}

% \bibitem{maker} P. D. Maker, R. W. Terhune, and C. M. Savage, Intensity-dependent changes in the refractive index of liquids. Physical Review Letters \textbf{12}, 507 (1964).


% \bibitem{Matsko} Matsko, A. B., Novikova, I., Welch, G. R., Budker, D., Kimball, D. F., and Rochester, S. M. Vacuum squeezing in atomic media via self-rotation. Physical Review A \textbf{66}, 043815  (2002).



% \bibitem{lvovskyselfrot} J. Ries, B. Brezger, and A. I. Lvovsky, Experimental vacuum squeezing in rubidium vapor via self-rotation, Physical Review A \textbf{68}, 025801 (2003).

% %\bibitem{Squeezing} Zhifei Yu, Shuqi Liu, Jinxian Guo, Guzhi Bao, Yuan Wu, and Liqing Chen, Enhancing vacuum squeezing via magnetic field optimization, Optics Express \textbf{30}, 17106-17114 (2022).

% \bibitem{Mikhailov} E. E. Mikhailov and I. Novikova, Low-frequency vacuum squeezing via polarization self-rotation in Rb vapor, Opt.
% Lett. \textbf{33}, 1213–1215 (2008).
% %\bibitem{OPO_overview} M. Martinelli, C. L. Garrido Alzar, P. H. Souto Ribeirox, and P. Nussenzveig, Classical and Quantum Properties of Optical Parametric Brazilian Journal of Physics \textbf{31(4)}, 597 (2001).


% %\bibitem{budkermain} S.M. Rochester, D.S. Hsiung, D. Budker, R.Y. Chiao, D.F. Kimball, and V.V. Yashchuk, Self-rotation of resonant elliptically polarized light in collision-free rubidium vapor, Phys. Rev. A \textbf{63}, 043814 (2001). 



% %\bibitem{FWMOPO1}R. H. Stolen and J. E. Bjorkholm, “Parametric amplification and frequency conversion in optical fibers,” IEEE J.
% Quantum Electron. \textbf{18}(7), 1062–1072 (1982).

% %\bibitem{FWMOPO2} N. Shibata, R. Braun, and R. Waarts, “Phase-mismatch dependence of efficiency of wave generation through four-wave mixing in a single-mode optical fiber,” IEEE J. Quantum Electron. \textbf{23}(7), 1205–1210 (1987). 

% %\bibitem{FWMOPO3} Jay E Sharping, Marco Fiorentino, Prem Kumar, Robert S Windeler, Optical parametric oscillator based on four-wave mixing in microstructure fiber, Opt. Lett. \textbf{27}, 1675 (2002).

% %\bibitem{lipson} Avik Dutt, {\it et al.,} On-Chip Optical Squeezing,  Phys. Rev. Applied \textbf{3}, 044005, (2015).


% \bibitem{Zheludev89}  N. I. Zheludev, ``Polarization instability and multistability in nonlinear optics" Sov. Phys. Usp. 32 357 (1989).

% \bibitem{Kerrcontroller} N. Moroney, {\it et. al.} A Kerr polarization controller, Nature Communications \textbf{13}, 398 (2022).


% %\bibitem{OPO_CIM} Marcello Calvanese Strinati, Leon Bello, Emanuele G. Dalla Torre, and Avi Pe’er, Can Nonlinear Parametric Oscillators Solve Random Ising Models? Phys. Rev. Lett. \textbf{126}, 143901 (2021).

% % \bibitem{Opt_Trist_Th} M. Kitano, T. Yabuzaki, and T. Ogawa, Optical Tristability. Physical Review Letters \textbf{46}, 926 (1980).

% % \bibitem{Opt_Trist_Exp} S. Cecchi, G. Giusfredi, E. Petriel, and P. Salieri, Observation of Optical Tristability in Sodium Vapors. Physical Review Letters \textbf{49}, 1928 (1982).

% % \bibitem{Bist_opo1} Lugovoi, V.N., Bistability and hysteresis phenomena in an optical parametric oscillator, Phys. stat. sol.(b),  \textbf{94}, 79-86 (1979).


% % \bibitem{Bist_opo2} C. Richy, K. I. Petsas, E. Giacobino, C. Fabre, and L. Lugiato, "Observation of bistability and delayed bifurcation in a triply resonant optical parametric oscillator," J. Opt. Soc. Am. B \textbf{12}, 456-461 (1995).


% % \bibitem{Bist_ker1} Hai  Wang, D. J. Goorskey, and Min Xiao, Bistability and instability of three-level atoms inside an optical cavity,
% % Phys. Rev. A \textbf{65}, 011801(R) (2001).

% % \bibitem{Bist_ker2} Hannes Gothe, Tristan Valenzuela, Matteo Cristiani, and Jürgen Eschner, Optical bistability and nonlinear dynamics by saturation of cold Yb atoms in a cavity, Phys. Rev. A \textbf{99}, 013849 (2019).

% %\bibitem{OpO_Chi2} Alexander W. Bruch, Xianwen Liu, Joshua B. Surya, Chang-Ling Zou, and Hong X. Tang, On-chip $\chi$(2) microring optical parametric oscillator. Optica \textbf{6(10)}, 1361-1366 (2019).
% %\bibitem{Yu2022} Zhifei Yu, Shuqi Liu, Jinxian Guo, Guzhi Bao, Yuan Wu, and Liqing Chen, Enhancing vacuum squeezing via magnetic field optimization, Opt. Express \textbf{30}, 17106--17114 (2022).

% \bibitem{rand1} T. Steinle, J. N. Greiner, J. Wrachtrup, H. Giessen, and I. Gerhardt,  Unbiased All-Optical Random-Number Generator, Phys. Rev. X \textbf{7}, 041050 (2017)

% \bibitem{rand2} L. Quinn, G. Xu, Y. Xu, Z. Li, J. Fatome, S. G. Murdoch, S. Coen, and M. Erkintalo, Random number generation using spontaneous symmetry breaking in a Kerr resonator, Opt. Lett. \textbf{48}, 3741-3744 (2023)




% % \bibitem{cim1} Wang, Z., Marandi, A., Wen, K., Byer, R. L. and Yamamoto, Y., Coherent Ising machine based on degenerate optical parametric oscillators. Physical Review A \textbf{88(6)}, 063853 (2013).

% % \bibitem{cim2} P. L. McMahon, {\it et al.,} A fully programmable 100-spin coherent Ising machine with all-to-all connections, Science \textbf{354(6312)}, 614-617 (2016).

% % \bibitem{cim3} Takahiro Inagaki, Kensuke Inaba, Ryan Hamerly, Kyo Inoue, Yoshihisa Yamamoto and Hiroki Takesue, Large-scale Ising spin network based on degenerate optical parametric oscillators, Nature Photonics \textbf{10}, 415–419 (2016).

% % \bibitem{cim4} D. Pierangeli, G. Marcucci, and C. Conti, Large-Scale Photonic Ising Machine by Spatial Light Modulation, Phys. Rev. Lett. \textbf{122}, 213902 (2019).

% % \bibitem{cim5} Fabian Böhm, Guy Verschaffelt and Guy Van der Sande, A poor man’s coherent Ising machine based on opto-electronic feedback systems for solving optimization problems, Nature Communications \textbf{10}, 3538 (2019).

% % \bibitem{cim6} Y. Yamamoto, T. Leleu, S. Ganguli, H. Mabuchi, Coherent Ising machines—Quantum optics and neural network Perspectives, Appl. Phys. Lett. \textbf{117}, 160501 (2020).

% % \bibitem{cim7} Toshimori Honjo, Tomohiro Sonobe, Kensuke Inaba, Takahiro Inagaki, Takuya Ikuta, Yasuhiro Yamada, Takushi Kazama, Koji Enbutsu, Takeshi Umeki, Ryoichi Kasahara, Ken-Ichi Kawarabayashi, Hiroki Takesue, 100,000-spin coherent Ising machine, Sci. Adv. \textbf{7} (2021).


% % \bibitem{cim8} Marcello Calvanese Strinati, Davide Pierangeli, and Claudio Conti, All-Optical Scalable Spatial Coherent Ising Machine, Physical Review Applied \textbf{16}, 054022 (2021).

% % \bibitem{cim9} Naeimeh Mohseni, Peter L. McMahon and Tim Byrnes, Ising machines as hardware solvers of combinatorial optimization problems, Nature Reviews Physics  \textbf{4}, 363–379 (2022).

% % \bibitem{cim10} Li Luo, Zhiyi Mi, Junyi Huang, and Zhichao Ruan, Wavelength-division multiplexing optical Ising simulator enabling fully programmable spin couplings and external magnetic fields, Science Advances \textbf{9(48)}, (2023).

% % \bibitem{cim11} Liam Quinn, Gang Xu, Yiqing Xu, Zongda Li, Julien Fatome, Stuart G. Murdoch, Miro Erkintalo, Stéphane Coen, Towards a novel coherent Ising machine using symmetry breaking in a Kerr resonator, AI and Optical Data Sciences IV; \textbf{PC1243806}, (2023).

% % \bibitem{Kerrcontroller} N. Moroney, {\it et. al.} A Kerr polarization controller, Nature Communications \textbf{13}, 398 (2022).

% %\bibitem{budkermain} S.M. Rochester, D.S. Hsiung, D. Budker, R.Y. Chiao, D.F. Kimball, and V.V. Yashchuk, Self-rotation of resonant elliptically polarized light in collision-free rubidium vapor, Phys. Rev. A \textbf{63}, 043814 (2001). 

% %\bibitem{nonlinfarad} D. Budker, W. Gawlik, D. F. Kimball, S. M. Rochester, V. V. Yashchuk, and A. Weis, Resonant nonlinear magneto-optical effects in atoms, Review of Modern Physics  \textbf{74}, 1153 (2002).

% %\bibitem{entangledimages} Vincent Boyer, Alberto M. Marino, Raphael C. Pooser, Paul D. Lett, Entangled Images from Four-Wave Mixing. Science \textbf{321}, 5888 (2008).

% \bibitem{nir} Vishwa Pal, Simon Mahler, Chene Tradonsky, Asher A. Friesem, and Nir Davidson, Rapid fair sampling of the XY spin Hamiltonian with a laser simulator. Phys. Rev. Research \textbf{2}, 033008 (2020).

% %\bibitem{scully} M. O. Scully and M. S. Zubairy, Quantum Optics (Cambridge University Press, 1997).

% \bibitem{polarizationbook} J. Peatross, M. Ware, Physics of Light and Optics (Brigham Young University, 2015). 


==> self_rot_old.tex <==
\subsection{Self rotation: theory}

Initially isotropic $\chi^3$ medium could become birefringent when exposed to elliptically polarized light. Two orthogonal components with circular polarizations differ in intensity, therefore experience different indices of refraction and propagate with dissimilar phase velocities. This effect was closely studied in atomic media. Mechanisms causing this, including an optical pumping, were revealed by \cite{budkermain}.

While propagating through a nonlinear media of length $l$, the polarization ellipse of light will rotate by an angle $\varphi$, in the first order proportional to ellipticity $\varepsilon \ll 1$:
\begin{equation}
   \varphi = g l \varepsilon 
   \label{eq:phi}
\end{equation}
where the rotation parameter g depends on intensity and frequency of the incident light. For a monochromatic slightly elliptically polarized light of frequency $\omega$, propagating in the $z$ direction, components of complex field amplitude can be described as $\mathcal{E}_H = X_H$ and $\mathcal{E}_V = X_V + i P_V$ with $\left|\mathcal{E}_V\right| \ll\left|\mathcal{E}_H\right|$. Under this assumption, $\mathcal{E}_H$ can be considered a "pump" field while $\mathcal{E}_V$ regarded as a probe field. Ellipticity $\varepsilon$ of such laser light is

\begin{equation}
\varepsilon = \mathrm{arctg}\dfrac{E_{min}}{E_{max}}\approx \frac{P_V(z)}{\mathcal{E}_H(z)}
\label{eq:ell}
\end{equation}

The self-rotation process leads to the following transformation of quadratures:

\begin{equation}
  \begin{cases}
    X_V(l)=X_V(0)+\varphi \mathcal{E}_H \approx X_V(0) + g l P_V(0)\\
    P_V(l)=P_V(0)
  \end{cases}
\label{quadratures}
\end{equation}
while $\mathcal{E}_H$ and $\varepsilon$ is unchanged in the first order \cite{lvovskyselfrot}.

However, to understand the dynamic of polarization self-rotation in a polarization selective resonator, it is important to determine polarization ellipse rotation angle and corresponding transformation of quadratures for all initial ellipticities, going beyond $\varepsilon \ll 1$.

Following the work \cite{budkermain}, we consider a 2-level system $J_g = 1/2 \rightarrow J_e = 1/2$. %as a simple model of self-rotation phenomena.
In such system, ground and exited levels are degenerate by magnetic quantum number $m$. According to the selection rules, transition $m_g = 1/2 \rightarrow m_e = -1/2$ can absorb only photons with left circular polarization, while $m_g = -1/2 \rightarrow m_e = 1/2$ absorbs only photons with right circular polarization, others transitions are forbidden.


\begin{figure}[ht!]
\center{\includegraphics[width =0.99\linewidth]{selfrot_img/Energy levels structure_3.pdf}}
\caption{Schematic diagram of energy levels with possible transitions}
\label{levels}
\end{figure}

We assume that the evolution of this system is determined by atom-light interaction via the rotating wave Hamiltonian and two kinds of spontaneous transitions within the atom, labeled as $\gamma$ and $\Gamma$ in Fig.\ref{levels}. Equation on a density matrix 

\begin{equation}
    \dot{\hat{\rho}}=-\dfrac{i}{\hbar}[\hat{H} ,\hat{\rho}]-\dfrac{1}{2}\{\hat{\Gamma}, \hat{\rho}\},
\end{equation}

where $\hat{\Gamma}$ is the relaxation matrix, $\hat{H}$ is the rotating wave Hamiltonian.

Solving Master equations (see Supplementary \ref{mastereq}), we obtain expressions for all elements of the density matrix $\hat{\rho}$, fully describing the stationary state of degenerate 2-level system. Refractive indices for polarization components can be obtained from $ \vec{P} = Tr(\hat{\rho} \hat{\vec{d}})$:

\begin{equation}
\begin{gathered}
n_{R} \sim
\dfrac{I_L \delta}{\left(1+4 \delta^2\right) I+4 \dfrac{I_R I_L}{I_{sat}}}
\end{gathered}
\label{eq:npl}
\end{equation}


\begin{equation}
\begin{gathered}
n_{L} \sim
\dfrac{I_R \delta}{\left(1+4 \delta^2\right) I+4 \dfrac{I_R I_L}{I_{sat}}},
\end{gathered}
\label{eq:nmin}
\end{equation}

where $I_{R, L}$ are intensities of right and left circularly polarized components respectively, $I$ is a full intensity of light, $I_{sat}$ is the saturation intensity, $\delta$ is the ratio of the resonance detuning to the resonance line width.


As can be seen from Eq.\ref{eq:npl} and Eq.\ref{eq:nmin}, birefringence of such system manifests itself only when intensities of left and right circular components are not equal. It leads to a non-zero phase shift between them 
%after the interaction with rubidium atoms
and results in the rotation of polarization by an angle $\varphi$ (see Supplementary \ref{mastereq} for more details):

\begin{equation}
\begin{gathered}
\varphi = - \frac{k l (n_R - n_L) }{2} \sim \\
\sim \dfrac{ \delta \sin(2 \varepsilon)}{(2 + 8 \delta^2) + (1 + \cos(4 \varepsilon))\dfrac{I}{I_{sat}}},
\end{gathered}
\label{eq:8}
\end{equation}

where $I$ is the intensity of input light, $I_{sat}$ is the saturation intensity,  $\delta = \Delta \slash (\Gamma + \gamma)$ is the ratio of frequency detuning to the line width.
%We theoretically investigated the dependence of the rotation angle of the polarization ellipse to be expected after the light passing through the rubidium cell on the initial ellipticity. A graph of this dependence is given in the next section, here we briefly describe its main characteristics.

%After that we theoretically calculated the dependence of the rotation angle of the polarization ellipse on the initial ellipticity to be expected after the light passing through the rubidium cell.

%Let us describe main features of this dependence. First of all, it is to be expected that the rotation angle of the polarization ellipse is zero with zero initial ellipticity. Secondly, With its increase, difference in refractive indices and relative phase shift for two orthogonal components increase as well (see Eq. \ref{eq:npl} and Eq. \ref{eq:nmin}). This will result in a more prominent rotation of the polarization ellipse meaning this function is a monotonically non-decreasing. 

%Now let us discuss an experimental measurements and compare it to discussed theoretical model.
\subsection{Self rotation: experiment}

\label{expselfrot}
\begin{figure}[h]

%убрать лямбда/4 после ячейки
\center{\includegraphics[width = 8.6 cm]{selfrot_img/selft rot sheme1.pdf}}
	\caption{Experimental setup for measuring the dependence of polarization ellipse rotation angle on the initial ellipticity. Laser radiation is focused into the cell containing rubidium vapour. A fine-adjustable $\lambda / 4$ plate in front of the cell is used to make initial horizontal polarization of a pump elliptical (see
text).}
	\label{ris:sr-scheme}
\end{figure}

%1st: provide a H-pol pump
A scheme of the experimental setup is shown in Fig.\ref{ris:sr-scheme}. The beam from an external cavity diode laser system (Vitawave ECDL-7950R) delivers approximately $50 \mathrm{~mW}$ of optical power in a single mode. The laser is tuned across the rubidium D1 line ($\lambda \simeq 795 \mathrm{~nm}$). The beam is shaped by a pair of lenses and then sent through a high quality Glan prism that transmits strictly linear polarisation. The wave plate is placed before the Glan prism to vary the pump intensity. Horizontally polarised light beam is then focused by a lens into a cylindrical vapour cell ($25 \mathrm{~mm}$ in diameter and $75 \mathrm{~mm}$ in length) filled with ${ }^{85} \mathrm{Rb}$.

%2nd: ell
To produce and control an ellipticity in the initially horizontally polarised beam, a fine-adjustable $\lambda / 4$ plate is placed in front of the cell. To compensate the impact of birefringent windows on pumping light, we align polarisation ellipse major axis with an optical axis of windows of vapour cell. To do it we place $\lambda / 2$ wave plate after $\lambda / 4$ and adjust it every time we rotate the $\lambda / 4$ plate.

%3rd: measurement
After exiting the cell, the beam is directed to the measuring system consisting of a $ \lambda /2$ wave plate and a PBS, whose axis is alligned with respect to the axis of the Glan prism. By rotating $ \lambda /2$ plate, we can measure signal in either canonical or diagonal basis. The outputs of the PBS are directed to two photodiodes (PD$_{1}$ and PD$_{2}$). Data is gathered by tuning the laser through rubidium D1 line for a range of initial ellipticities and recording the signal from the photodiodes.

Let $I_{H}$ and $I_{V}$ be signals on photodiodes $\mathrm{PD_{1}}$ and $\mathrm{PD_{2}}$ respectively while measuring in canonical basis. These values correspond to intensity of horizontally and vertically polarised light, emerging from the vapour cell.

Similarly, we denote signals obtained while measuring in diagonal basis by $I_{+}$ and $I_{-}$, so they correspond to intensity of linearly polarised light at angles $\pm 45^{\circ}$ to horizontal.

Calculations show that a rotation angle of polarisation ellipse is determined by

\begin{equation}
    \varphi = \dfrac{1}{2}\mathrm{arctan}\Big(\dfrac{I_{+} - I_{-}}{I_{+} + I_{-} - 2I_{V}}\Big)
\label{eq:selfrot_formula}
\end{equation}

For derivation of the equation above see Supplementary \ref{derivation}.

Figure \ref{fig:gl} shows polarisation self-rotation parameter $gl$ for a small initial ellipticity and coefficient of absorption $\alpha l$ for zero ellipticity measured near the D1 line of ${ }^{85} \mathrm{Rb}$.
$gl$ was determined using equations \ref{eq:phi}, \ref{eq:selfrot_formula}. 
Coefficient of absorption $\alpha l$ is defined as $\alpha l = \ln{\left(I_{max}/I\right)}$, where $I_{max}$ corresponds to light intensity far from resonance.

\begin{figure}[ht!]
\center{\includegraphics[width = 0.99 \linewidth]{selfrot_img/gl.pdf}}
\caption{Polarisation self-rotation parameter $gl$ (blue line, left scale) and coefficient of absorption $\alpha l$ (red line, right scale) measured across the ${ }^{85} \mathrm{Rb}$ D1 transition at $70^{\circ}\mathrm{C}$. Zero detuning corresponds to maximum absorption and, therefore, to exact frequency of D1 transition in ${ }^{85} \mathrm{Rb}$. Green region marks the frequency range where bistability were observed. Bistability presents only in a narrow frequency range with the lowest losses and the highest non-linearity. Here and below frequency was calibrated by the spectroscopy signal from reference Rb cell with input power P = 44 $\mu$W at temperature $22^{\circ}$C}.
\label{fig:gl}
\end{figure}

Working temperature is $70^{\circ}\mathrm{C}$, pump power is approximately $14 \mathrm{~mW}$. With an estimated focal beam diameter of $50 \,\mu\mathrm{m}$, we experimentally obtain $I_{sat} \simeq 0.8 \mathrm{~mW}$, thus operating in a high saturation regime. As it can be seen in Fig. \ref{fig:colorP1}, the dependence $\varphi(\varepsilon)$ is independent from pump power across the range [1 mW, 14.5 mW]. If the pump power is below 0.5 mW, then the frequency profile of the effect (see Fig. \ref{fig:gl}) becomes asymmetrical, which may indicate an interference of some other phenomena. Since we do not use any kind of magnetic shielding, this phenomenon might be a non-linear Faraday rotation \cite{nonlinfarad}. We suppose it because the frequency profile of self-rotation is expected to be symmetrical on the D1 rubidium line \cite{budkermain}.

\begin{figure}[ht!]
\center{\includegraphics[width = 0.99 \linewidth]{selfrot_img/color I small e.pdf}}
\caption{Dependence of ellipse rotation angle $\varphi$ on pump power $P$ and frequency detuning $\Delta$ with fixed ellipticity $\varepsilon = 0.035$. Value of $\varphi$ in rad is coded by color.}
\label{fig:colorP1}
\end{figure}

An ellipticity produced by the $\lambda/4$ wave plate is equal to rotation angle of the named plate (in rad). So we investigate a polarisation ellipse rotation for angles of the $\lambda / 4$ plate in range 0-45 degrees. Experimental results are presented in Fig.\ref{fig:phi_eps}.

\begin{figure}[ht!]
\center{\includegraphics[width = 0.99 \linewidth]{selfrot_img/phi(eps).pdf}}
\caption{Dependence of polarisation ellipse rotation angle on initial ellipticity at fixed pump power $P = 13.5$ mW and frequency detuning $\Delta = 0.35$ GHz. Experimental data (blue dots) is compared to the theoretically obtained curve (red line) from Eq.\ref{eq:8}.}
\label{fig:phi_eps}
\end{figure}

As can be seen from the figure, the rotation angle of polarisation ellipse is zero with zero initial ellipticity and it increases monotonously, which is consistent with the theory.
%Experiment is qualitatively consistent with the theory. 

The full dependence $\varphi(\varepsilon, \; \Delta)$ is presented in Fig. \ref{fig:color2}.

\begin{figure}[ht!]
\center{\includegraphics[width = 0.99 \linewidth]{selfrot_img/color2.pdf}}
\caption{Dependence of ellipse rotation angle $\varphi$ on ellipticity $\varepsilon$ and frequency detuning $\Delta$ while pump power is fixed $P = 13.5$ mW. The value of $\varphi$ in rad is illustrated by color.}
\label{fig:color2}
\end{figure}


The numerical difference can be attributed to imperfection of our theory. In reality energy levels structure of rubidium atoms is more complex then a 4-level system.
